Robot-to-Robot Relative Pose Estimation using Humans as Markers

In this paper, we propose a method to determine the 3D relative pose of pairs of communicating robots by using human pose-based key-points as correspondences. We adopt a 'leader-follower' framework, where at first, the leader robot visually detects and triangulates the key-points using the state-of-the-art pose detector named OpenPose. Afterward, the follower robots match the corresponding 2D projections on their respective calibrated cameras and find their relative poses by solving the perspective-n-point (PnP) problem. In the proposed method, we design an efficient person re-identification technique for associating the mutually visible humans in the scene. Additionally, we present an iterative optimization algorithm to refine the associated key-points based on their local structural properties in the image space. We demonstrate that these refinement processes are essential to establish accurate key-point correspondences across viewpoints. Furthermore, we evaluate the performance of the proposed relative pose estimation system through several experiments conducted in terrestrial and underwater environments. Finally, we discuss the relevant operational challenges of this approach and analyze its feasibility for multi-robot cooperative systems in human-dominated social settings and feature-deprived environments such as underwater.

==> srctex/appen.tex <==

\newpage

\subsection*{Appendix I: Two-view structure from motion}
\begin{figure*}[h]
	\centering
	\begin{subfigure}{0.49\textwidth}
		\centering	
		\includegraphics[width=\linewidth]{figs/appen1a.pdf}
		\caption{Three humans seen from two different views.}
	\end{subfigure}~
	\begin{subfigure}{0.49\textwidth}
		\centering	
		\includegraphics[width=\linewidth]{figs/appen1b.pdf}
		\caption{Key-point correspondences and epipolar lines.}
	\end{subfigure}
	\vspace{3mm}
	
	\begin{subfigure}{\textwidth}
		\centering	
		\includegraphics[width=\linewidth]{figs/appen1c.pdf}
		\caption{The reconstructed 3D key-points and the estimated camera poses (up-to scale).}
	\end{subfigure}
	\vspace{3mm}
	
	\begin{subfigure}{0.49\textwidth}
	\centering	
	\includegraphics[width=\linewidth]{figs/appen1d.pdf}
	\caption{Reduction of the average re-projection error by the iterative key-point refinement process.}
    \end{subfigure}~
	\begin{subfigure}{0.47\textwidth}
	\centering	
	\includegraphics[width=\linewidth]{figs/6a.jpg}
	\caption{Re-projected points (red crosses) on the left image are shown; the blue circles represent true locations.}
    \end{subfigure}
    

\caption{\emph{Structure from motion} for a \emph{two-view} case using only human pose-based key-points as features.}
\label{fig:appen1}
\end{figure*}
\newpage


\subsection*{Appendix II: Performance of the proposed person ReId method}
\begin{figure*}[h]
	\centering
	\begin{subfigure}{\textwidth}
		\centering	
		\includegraphics [width=0.48\linewidth]{figs/b0.png} 
		\includegraphics [width=0.482\linewidth]{figs/b1.png} 
		\caption{Ground scenario: with occlusion and considerable pose changes.}
	\end{subfigure}
		\vspace{2mm}
		
		
		\begin{subfigure}{\textwidth}
		\centering	
		\includegraphics [width=0.45\linewidth]{figs/combo_n1.png} 
		\includegraphics [width=0.52\linewidth]{figs/combo_n3.png}
		\caption{Underwater scenario: with occlusion and considerable pose changes.}
	\end{subfigure}
	
    \caption{A few sample results for the proposed person ReId method; it assigns an unique identifier for each association.}
\label{fig:reid}
\end{figure*}
